Time Series Forecasting with Hypernetworks Generating Parameters in Advance

Forecasting future outcomes from recent time series data is not easy, especially when the future data are different from the past (i.e. time series are under temporal drifts). Existing approaches show limited performances under data drifts, and we identify the main reason: It takes time for a model to collect sufficient training data and adjust its parameters for complicated temporal patterns whenever the underlying dynamics change. To address this issue, we study a new approach; instead of adjusting model parameters (by continuously re-training a model on new data), we build a hypernetwork that generates other target models' parameters expected to perform well on the future data. Therefore, we can adjust the model parameters beforehand (if the hypernetwork is correct). We conduct extensive experiments with 6 target models, 6 baselines, and 4 datasets, and show that our HyperGPA outperforms other baselines.

==> sections/abstract.sh.tex <==


% --------------------------------------------------------------------------------
%   Abstract
% --------------------------------------------------------------------------------
\begin{abstract}
%
Models forecasting future outcomes from time series data require the ability to \emph{extrapolate} from previous observations.
%
Yet, this extrapolation is not easy, especially when a model is under data drift, \textit{e.g.}, the future outcomes are different from the past.
%
Existing approaches show limited performances under data drifts, and we identify the main reason:
% \textcolor{green}{models can forecast for the future in the range of the past data.}
% \textcolor{red}{it takes time for a model to \emph{adjust} its parameters for complicated temporal patterns.}
It takes time for a model to collect sufficient training data and \emph{adjust} its parameters for complicated temporal patterns whenever the underlying dynamics change.
%
To address this issue, we study a new approach; 
%
instead of adjusting model parameters (by continuously re-training a model on new data), we build a \emph{meta-model} (or \emph{hypernetwork}) that generates other target models' parameters expected to perform well on the future data. Therefore, we can adjust the model parameters beforehand (if the meta-model is correct).
%
We conduct extensive experiments with 6 target models, 4 baselines, and 4 datasets, and show that our \textit{HyperGPA} outperforms other baselines.
%
% \SH{Explain how we train HyperGPA; what are the major technical advances?}

%
% \SH{Mention some more about the ablation study, etc.}
%
\end{abstract}


==> sections/intro.save.tex <==



\section{Introduction}
\begin{figure}[!ht]
    \centering
    \subfigure[An example of weekly time series data (the U.S. flu dataset) where each year constitutes a temporal window]{\includegraphics[width=\columnwidth]{fig/time_series.pdf}}
    \subfigure[Conventional approach where models are updated every window. Depending on cases, we can maintain only one model or multiple models for those $M$ time series (The depicted is a multi-model example in this figure).]{\includegraphics[width=\columnwidth]{fig/existing.pdf}}
    \subfigure[Proposed approach where parameters $\{\hat{\theta}_{i,4}\}_{i=1}^M$ are forecast]{\includegraphics[width=\columnwidth]{fig/HyperGPA.pdf}}
    \caption{A comparison between a conventional approach and our proposed approach. (a) The U.S. flu dataset contains influenza-like illness time series data. (b) Each model is trained with a time series of past data and is used to forecast the future. (c) Our hypernetwork forecasts the future model parameters.}
    \label{fig:archi}
\end{figure}

Time series forecasting is one of the most fundamental problems in deep learning, ranging from classical climate~\citep{debrouwer2019gruodebayes,REN2021100178} and stock price forecasting~\citep{7046047,VIJH2020599} to recent pandemic forecasting~\citep{wu2020deep,pmlr-v144-wang21a}. Since these tasks are important in many real-world applications, diverse methods have been proposed, such as recurrent neural networks (RNNs~\citep{lstm,cho2014learning}), neural ordinary differential equations (NODEs~\citep{chen2019neural}), neural controlled differential equations (NCDEs~\citep{kidger2020neural}), and so on. Owing to these novel models, forecasting accuracy has been significantly enhanced over the past several years.

% Forecasting requires the ability to \emph{extrapolate}, \textit{i.e.}, networks should be able to learn latent patterns from the past observations and project the most probable patterns into the future.
%
However, this forecasting is challenging, especially when \emph{temporal} drifts exist in time series data (cf. Section~\ref{sec:motivation}), i.e., an underlying dynamics that produce temporal observations changes~\citep{10.5555/3042817.3043028,Oh2019RelaxedPS,DBLP:journals/corr/abs-2111-03422,anonymous2022reversible}. For example, in epidemics, it is often to observe a sudden outbreak of diseases. % {\color{red}However, it is occasionally challenging to forecast highly varying time series (cf. Sec~\ref{sec:mot}).} In this paper, therefore, we further enhance them by proposing an approach generating parameters ahead using a hypernetwork, called \emph{HyperGPA}.
To this end, we propose a new approach that enables highly accurate time series forecasting under dynamics (or distribution) drift.
%
Specifically, we present \emph{HyperGPA}, a hypernetwork generating parameters ahead. 
%
% Sanghyun: I reviewed from this point; will continue some time later; feel free to modify.
In usual settings, we train a model with historical data and use it to forecast the future (cf. Fig.~\ref{fig:archi} (b)). However, our approach is to \emph{forecast} neural network parameters that are expected to work well in the future (cf. Fig.~\ref{fig:archi} (c)).


% (a) One can periodically update the model parameters every time window and forecast for the next window. \textcolor{green}{(b) Similarly, our hypernetwork is trained with a time series of past model parameters, e.g., $\{\theta_i\}_{i=1}^3$ in the figure, and forecasts the future model parameters, e.g., $\theta_4$.}}

For our discussion, suppose the time series data at Fig.~\ref{fig:archi} (a) and there exists a time series forecasting model for each of the $M$ loosely coupled time series. For instance, the U.S. flu dataset contains the weekly reports of (the number of flu patients, the number of total patients, the number of total information providers) for each state, which constitutes 51 loosely coupled time series.

Hypernetworks are neural networks generating other neural networks' parameters~\citep{ha2016hypernetworks,pawlowski2018implicit,vonoswald2020continual,zhang2019anodev2}. In this work, our hypernetwork has two parts: one reads the past data of $M$ loosely coupled time series and generates hidden representations, and the other generates a set of parameters for each of the $M$ forecasting models (cf. Fig.~\ref{fig:archi2}). The key task in the first part is to forecast the future data characteristics from the past data characteristics, whereas the second part is to forecast the parameters that are expected to work well for the forecast future data characteristics.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{fig/HyperGPA2.pdf}
    \caption{The detailed architecture of \emph{HyperGPA}, where the first shared multi-task layer understands the past data patterns $\{\{\mathcal{D}_{i,j}\}_{j=1}^3\}_{i=1}^M$ and forecasts the future data patterns, and the second layer forecasts the model parameters that are expected to work well for the future data patterns. The gradients flow from the mean square error (MSE) loss between the ground-truth of $\{\mathcal{D}_{i,4}\}_{i=1}^M$ and their forecast values to the two layers. In other words, \emph{HyperGPA} is trained to output the target model's parameters that minimizes the task loss.}
    \label{fig:archi2}
\end{figure}

The first part of our hypernetwork can be understood as a \emph{shared multi-task} layer since it processes all the $M$ time series simultaneously for the second part which generates the parameters for each of those $M$ forecasting models. The shared layer i) reads $\{\{\mathcal{D}_{i,j}\}_{j=N-K}^{N-1}\}_{i=1}^M$, where $\mathcal{D}_{i,j}$ means a set of observations of the $i$-th time series in the $j$-th window (cf. Def.~\ref{def:window}), during the past $K$ windows for the $M$ loosely-coupled time series and ii) forecasts a vector that represents the data characteristics in the next window $\{\mathcal{D}_{i,N}\}_{i=1}^M$. For this part, we utilize recent graph convolutional network (GCN) and neural controlled differential equation (NCDE) technologies~\citep{bai2020adaptive,kidger2020neural}. GCNs are a representative spatial processing method and NCDEs are a recent breakthrough in processing time series.

% \textcolor{green}{In general, the same type of time-series data occurs in many places, simultaneously. They can have some relationships, for example, pandemic data in each state of USA. Therefore, reading the past data and forecasting the future data is a spatiotemporal forecasting task.

Similarly, the second part is also based on GCNs. Target neural network models are typically represented by computation graphs, and a parameter is interconnected with other parameters given a computation graph. Using this property, the second part, which utilizes a graph convolutional technique, forecasts the future parameters.

% To sum up, We design the hypernetwork using recent graph convolutional network (GCN) and neural controlled differential equation (NCDE) technologies. GCNs are a representative spatial processing method and NCDEs are a recent breakthrough in processing time series. By carefully integrating them, we can design our hypernetwork, a spatiotemporal neural network generating target model's parameters.



% our hypernetwork has  is a \emph{spatiotemporal} neural network that reads data $\{D_i\}_{i=N-K}^{N-1}$ during the past $K$ windows and forecasts the next parameter $\theta_N$.
%neural networks are represented by computation graphs, and a parameter is interconnected with other parameters given a neural network. 

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{fig/toy_ver2.pdf}
%     \caption{(upper figure) We use the sinusoidal signal whose amplitude gradually increases as time goes by. The green is a training line, and the grey is a testing line. We use a single-layer GRU network as a target forecasting model. (lower figure) A conventional approach, denoted `\textit{(W/O Hyper)}', doesn't catch the increasing amplitude. However, the target model whose parameters are generated by \emph{HyperGPA} is almost correct --- the mean squared error (MSE) of the conventional approach is 0.49 vs. 0.02 by \emph{HyperGPA}.}\label{fig:toy}
% \end{figure}

% In Fig.~\ref{fig:toy}, we compare the conventional approach in Fig.~\ref{fig:archi} (b) and the proposed \emph{HyperGPA} in Fig.~\ref{fig:archi} (c) with a toy data. For this toy experiment, we use a single-layer GRU network as a target model. The toy data consists of sinusoidal signal whose amplitude increases over time. So training (past) patterns are different from testing (future) patterns. In the baseline approach, the amplitude of the prediction, highlighted with dashed red, is smaller than that of the ground truth. However, the target model, whose parameters are configured by \emph{HyperGPA}, forecasts the almost same line as the true one, achieving a lower mean squared error (MSE).

We conduct experiments with 6 target time series forecasting models, 4 baselines, and 4 datasets. In particular, we show that our proposed hypernetwork-based approach can be successfully applied to almost all existing popular time series forecasting models, ranging from RNNs and NODEs to NCDEs, which is a significant enhancement in comparison with other hypernetwork approaches in~\citep{ha2016hypernetworks,zhang2019anodev2} which assume a certain target model type. Our method enhances the mean squared error of the target models up to 47.5\% in our experiments whereas existing hypernetwork-based approaches enhance them up to 22.6\%. Our contributions can be summarized as follows:
\begin{enumerate}
    \item We propose a hypernetwork, called \emph{HyperGPA}, that can forecast the future model parameters of various time series forecasting models.
    \item \emph{HyperGPA} can be applied to almost all existing popular time series forecasting models, ranging from RNNs/LSTMs/GRUs to NODEs/NCDEs.
    \item \emph{HyperGPA} enhances the target models' accuracy up to 47.5\% with 60\% smaller parameter numbers in comparison with the best performing baseline.
\end{enumerate}


% In many real-world applications, predicting the future data is 
% necessary, e.g., stock forecasting, weather forecasting, traffic forecasting, infectious disease forecasting\colorbox{green}{~\ref{}}, and so on. One of the ways solving this problem is the neural network, and many time-series neural networks have proliferated. \colorbox{green}{~\ref{}}. 

% In general, for time-series training neural networks, the sliding window approach is applied, Fig.~\ref{fig:sliding_window}. Given data $x_t$ indexed by time $t$, and input/output window size $w_{in}$,$w_{out}$, input $X$ is $\{x_{t},x_{t+1},...,x_{t+w_{in}-1}\}$, and output $Y$ is $\{x_{t+w_{in}},x_{t+w_{in}+1},...,x_{t+w_{in}+w_{out}-1}\}$. Using the past data before time $T$, the neural network learns the output pattern according to the input pattern. Because output and input length ($w_{in}, w_{out}$) is fixed, all batches have same length and the neural network is trained more easily. After training, the neural network forecasts unseen data recursively. It predicts $\{x_{T},x_{},...,x_{T+w_{out}-1}\}$ with $w_{in}$ length input data right before T, predicts next time sequence using the predicted data, $\{x_{T},x_{},...,x_{T+w_{out}-1}\}$, and goes on.
% \begin{figure}
% \centering
% \includegraphics[width=0.9\columnwidth]{fig/sliding window.pdf}
% \caption{Sliding Window Approach}
% \label{fig:sliding_window}
% \end{figure}


% There are various time-series models ranging from recurrent neural network (RNNs) to sequence-to-sequence model (SeqToSeqs), and neural ordinary/controlled differential equations (NODEs and NCDEs). NODE/NCDE can process irregular time-series data, whereas others can process regular that. As the new models are proposed, forecasting performance gradually increases. However, there is the natural limitation. The limitation is that the neural network forecasts $Y$ with $X$ only when train data contains the data similar to $(X,Y)$ pair. If train data is $(X,Y)$ and test data is $(X,Y')$, where $Y'$ is significantly different with $Y$, the neural network never forecasts $Y'$ with $X$. In real-word data, the different patterns between the past and future data occurs frequently.\colorbox{green}{\ref{}}  
% Increasing $w_{in}$ can be a solution, but too large $w_{in}$ can make training unstable \colorbox{green}{\ref{}}.

% To this end, we propose this model, \underline{\textbf{Hyper}}network \underline{\textbf{G}}enerating \underline{\textbf{P}}aramter \underline{\textbf{A}}head (Hyper-GPA).


